On the Existence of Cyclic Lattice Codes

A coding lattice $\Lambda_c$ and a shaping lattice $\Lambda_s$ forms a nested lattice code $\mathcal{C}$ if $\Lambda_s \subseteq \Lambda_c$. Under some conditions, $\mathcal{C}$ is a finite cyclic group formed by rectangular encoding. This paper presents the conditions for the existence of such $\mathcal{C}$ and provides some designs. These designs correspond to solutions to linear Diophantine equations so that a cyclic lattice code $\mathcal C$ of arbitrary codebook size $M$ can possess group isomorphism, which is an essential property for a nested lattice code to be applied in physical layer network relaying techniques such as compute and forward.

==> figures/nested.tex <==
\definecolor{gray}{rgb}{0.7,0.7,0.7}
\definecolor{niceBlue}{rgb}{0,    0.2824,    0.6314}
\definecolor{niceRed}{rgb}{0.7686,    0.0078,    0.0078}
\scalebox{0.45}{
\begin{tikzpicture}[>=latex]
Clip to a window
\clip (-5.5,-5.5) rectangle (5.5,5.5);  
%draw the x grid lines and labels
\foreach \i in {0} {
   \draw[domain=-6:6, smooth, variable=\y, gray]  plot (\i, {\y});
}
%draw the y grid lines and labels
\foreach \i in {0} {
   \draw[domain=-4:7, smooth, variable=\y, gray]  plot ({\y},\i);
}
%See latticeCodingTheory/figs/matlab/shapingRegion
%lattice points
\foreach \i/\j in {
0/0, 0/1, 0/2, 0/3, 0/-3, 0/-2, 0/-1, 0.87/0.5, 0.87/1.5, 0.87/2.5, 0.87/-3.5, 0.87/-2.5, 0.87/-1.5, 0.87/-0.5, 1.73/1, 1.73/2, 1.73/3, 1.73/-3, 1.73/-2, 1.73/-1, 1.73/0, 2.6/1.5, 2.6/-1.5, 2.6/-0.5, 2.6/0.5, 3.46/0, -3.46/-1, -3.46/0, -3.46/1, -2.6/-1.5, -2.6/-0.5, -2.6/0.5, -2.6/1.5, -2.6/2.5, -2.6/-2.5, -1.73/-1, -1.73/0, -1.73/1, -1.73/2, -1.73/3, -1.73/-3, -1.73/-2, -0.87/-0.5, -0.87/0.5, -0.87/1.5, -0.87/2.5, -0.87/-3.5, -0.87/-2.5, -0.87/-1.5
} {
        \fill (\i,\j) circle (0.1) [fill=niceBlue]; 
}
\foreach \i/\j in {
0/4, 0/5, 0/-5, 0/-4, 0.87/3.5, 0.87/4.5, 0.87/-4.5, 1.73/4, 1.73/5, 1.73/-5, 1.73/-4, 2.6/2.5, 2.6/3.5, 2.6/4.5, 2.6/-4.5, 2.6/-3.5, 2.6/-2.5, 3.46/2, 3.46/3, 3.46/4, 3.46/5, 3.46/-5, 3.46/-4, 3.46/-3, 3.46/-2, 3.46/-1, 3.46/1, 4.33/2.5, 4.33/3.5, 4.33/4.5, 4.33/-4.5, 4.33/-3.5, 4.33/-2.5, 4.33/-1.5, 4.33/-0.5, 4.33/0.5, 4.33/1.5, 5.2/3, 5.2/4, 5.2/5, 5.2/-5, 5.2/-4, 5.2/-3, 5.2/-2, 5.2/-1, 5.2/0, 5.2/1, 5.2/2, -5.2/-3, -5.2/-2, -5.2/-1, -5.2/0, -5.2/1, -5.2/2, -5.2/3, -5.2/4, -5.2/5, -5.2/-5, -5.2/-4, -4.33/-2.5, -4.33/-1.5, -4.33/-0.5, -4.33/0.5, -4.33/1.5, -4.33/2.5, -4.33/3.5, -4.33/4.5, -4.33/-4.5, -4.33/-3.5, -3.46/-2, -3.46/2, -3.46/3, -3.46/4, -3.46/5, -3.46/-5, -3.46/-4, -3.46/-3, -2.6/3.5, -2.6/4.5, -2.6/-4.5, -2.6/-3.5, -1.73/4, -1.73/5, -1.73/-5, -1.73/-4, -0.87/3.5, -0.87/4.5, -0.87/-4.5
} {
        \fill (\i,\j) circle (0.1) [fill=gray]; 
}
%\draw[thick,draw=niceRed] (4.04,0) -- (2.02,3.5) -- (-2.02,3.5) -- (-4.04,0) -- (-2.02,-3.5) -- (2.02,-3.5) -- (4.04,-0);
\draw[thick,draw=niceRed] (-2.02,3.5) -- (-4.04,0) -- (-2.02,-3.5) -- (2.02,-3.5);
\draw[thick,draw=niceRed] (-2.02,10.5) -- (-4.04,7) -- (-2.02,3.5) -- (2.02,3.5);
\draw[thick,draw=niceRed] (-2.02,-3.5) -- (-4.04,-7) -- (-2.02,-10.5) -- (2.02,-10.5);
\draw[thick,draw=niceRed] (4.04,7) -- (2.02,3.5) -- (4.04,0) -- (8.08,0);
\draw[thick,draw=niceRed] (-14.14,3.5) -- (-16.16,0) -- (-14.14,-3.5) -- (-10.1,-3.5);
\draw[thick,draw=niceRed] (4.04,0) -- (2.02,-3.5) -- (4.04,-7) -- (8.08,-7);
\draw[thick,draw=niceRed] (-8.08,0) -- (-10.1,-3.5) -- (-8.08,-7) -- (-4.04,-7);
\draw[thick,draw=niceRed] (-8.08,7) -- (-10.1,3.5) -- (-8.08,0) -- (-4.04,0);
\draw[thick,draw=niceRed] (-8.08,-7) -- (-10.1,-10.5) -- (-8.08,-14) -- (-4.04,-14);
\node [anchor=south west,color=niceBlue] at (0,0) {\Huge $\mathcal C$};
\end{tikzpicture}
}

==> figures/parallelogram.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.50196,0.50196,0.50196}%
\definecolor{mycolor2}{rgb}{0.76863,0.00784,0.00784}%
\definecolor{mycolor3}{rgb}{0.86670,0.96860,0.64710}%
\definecolor{mycolor4}{rgb}{0.55686,0.58824,0.47059}%
\definecolor{mycolor5}{rgb}{0.79216,0.70588,0.30980}%
\definecolor{mycolor6}{rgb}{0.38431,0.62353,0.50588}%
\definecolor{mycolor7}{rgb}{0.29804,0.33725,0.30588}%
\definecolor{mycolor8}{rgb}{0.68235,0.25882,0.09412}%
\definecolor{mycolor9}{rgb}{0.00000,0.49804,0.00000}%
\definecolor{mycolor10}{rgb}{0.00000,0.28235,0.63137}%
\definecolor{mycolor11}{rgb}{1.00000,0.49804,0.00000}%
\definecolor{mycolor12}{rgb}{0.90000,0.10000,0.60000}%
\definecolor{mycolor13}{rgb}{0.00000,0.50000,0.70000}%
%
\scalebox{0.7}{
\begin{tikzpicture}[%
scale=1
]

\begin{axis}[%
width=6.379cm,
height=9.814cm,
at={(0cm,0cm)},
scale only axis,
unbounded coords=jump,
xmin=-4.5,
xmax=9,
xtick={-5, -4, -3, -2, -1,  0,  1,  2,  3,  4,  5,  6,  7,  8,  9},
ymin=-4.42307692307692,
ymax=16.3461538461538,
ytick={-4, -3, -2, -1,  0,  1,  2,  3,  4,  5,  6,  7,  8,  9, 10, 11, 12, 13, 14, 15, 16},
axis background/.style={fill=white}
]
\addplot [color=mycolor1,mark size=1.8pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0	0\\
0	8\\
0	16\\
0	24\\
0	-8\\
4	4\\
4	12\\
4	20\\
4	28\\
4	-4\\
8	8\\
8	16\\
8	24\\
8	-8\\
8	0\\
12	12\\
12	20\\
12	28\\
12	-4\\
12	4\\
16	16\\
16	24\\
16	-8\\
16	0\\
16	8\\
-8	-8\\
-8	0\\
-8	8\\
-8	16\\
-8	24\\
-4	-4\\
-4	4\\
-4	12\\
-4	20\\
-4	28\\
};
\addplot [color=mycolor1,solid,forget plot]
  table[row sep=crcr]{%
0	4\\
0	4\\
nan	nan\\
0	12\\
0	12\\
nan	nan\\
0	20\\
0	20\\
nan	nan\\
0	-4\\
0	-4\\
nan	nan\\
4	0\\
0	4\\
nan	nan\\
0	4\\
4	8\\
nan	nan\\
4	8\\
0	12\\
nan	nan\\
0	12\\
4	16\\
nan	nan\\
4	8\\
4	8\\
nan	nan\\
4	16\\
0	20\\
nan	nan\\
0	20\\
4	24\\
nan	nan\\
4	16\\
4	16\\
nan	nan\\
4	24\\
0	28\\
nan	nan\\
4	24\\
4	24\\
nan	nan\\
0	-4\\
4	0\\
nan	nan\\
4	-8\\
0	-4\\
nan	nan\\
4	0\\
4	0\\
nan	nan\\
8	4\\
4	8\\
nan	nan\\
4	8\\
8	12\\
nan	nan\\
8	12\\
4	16\\
nan	nan\\
4	16\\
8	20\\
nan	nan\\
8	12\\
8	12\\
nan	nan\\
8	20\\
4	24\\
nan	nan\\
4	24\\
8	28\\
nan	nan\\
8	20\\
8	20\\
nan	nan\\
4	-8\\
8	-4\\
nan	nan\\
4	0\\
8	4\\
nan	nan\\
8	-4\\
4	0\\
nan	nan\\
8	4\\
8	4\\
nan	nan\\
8	-4\\
8	-4\\
nan	nan\\
12	8\\
8	12\\
nan	nan\\
8	12\\
12	16\\
nan	nan\\
12	16\\
8	20\\
nan	nan\\
8	20\\
12	24\\
nan	nan\\
12	16\\
12	16\\
nan	nan\\
12	24\\
8	28\\
nan	nan\\
12	24\\
12	24\\
nan	nan\\
12	-8\\
8	-4\\
nan	nan\\
8	-4\\
12	0\\
nan	nan\\
8	4\\
12	8\\
nan	nan\\
12	0\\
8	4\\
nan	nan\\
12	8\\
12	8\\
nan	nan\\
12	0\\
12	0\\
nan	nan\\
16	12\\
12	16\\
nan	nan\\
12	16\\
16	20\\
nan	nan\\
16	20\\
12	24\\
nan	nan\\
12	-8\\
16	-4\\
nan	nan\\
16	-4\\
12	0\\
nan	nan\\
12	0\\
16	4\\
nan	nan\\
12	8\\
16	12\\
nan	nan\\
16	4\\
12	8\\
nan	nan\\
-4	0\\
0	-4\\
nan	nan\\
0	-4\\
-4	-8\\
nan	nan\\
-4	-8\\
-8	-4\\
nan	nan\\
-8	-4\\
-4	0\\
nan	nan\\
0	4\\
-4	0\\
nan	nan\\
-4	8\\
0	4\\
nan	nan\\
-4	0\\
-8	4\\
nan	nan\\
-8	4\\
-4	8\\
nan	nan\\
-4	0\\
-4	0\\
nan	nan\\
0	12\\
-4	8\\
nan	nan\\
-4	16\\
0	12\\
nan	nan\\
-4	8\\
-8	12\\
nan	nan\\
-8	12\\
-4	16\\
nan	nan\\
-4	8\\
-4	8\\
nan	nan\\
0	20\\
-4	16\\
nan	nan\\
-4	24\\
0	20\\
nan	nan\\
-4	16\\
-8	20\\
nan	nan\\
-8	20\\
-4	24\\
nan	nan\\
-4	16\\
-4	16\\
nan	nan\\
0	28\\
-4	24\\
nan	nan\\
-4	24\\
-4	24\\
nan	nan\\
4	-8\\
4	-69.2666153055679\\
nan	nan\\
0	28\\
0	89.7057042201536\\
nan	nan\\
12	-8\\
12	-70.9643309091601\\
nan	nan\\
8	28\\
8	89.7057042201536\\
nan	nan\\
16	20\\
74.8871146573812	20\\
nan	nan\\
12	24\\
53.9958713325481	65.9958713325481\\
nan	nan\\
16	-4\\
77.7057042201536	-4\\
nan	nan\\
16	4\\
72.6830231705666	4\\
nan	nan\\
16	12\\
71.4321403661643	12\\
nan	nan\\
-4	-8\\
-4	-70.9643309091601\\
nan	nan\\
-8	-4\\
-69.7057042201536	-4\\
nan	nan\\
-8	4\\
-64.6830231705666	4\\
nan	nan\\
-8	12\\
-63.4321403661643	12\\
nan	nan\\
-8	20\\
-66.8871146573812	20\\
nan	nan\\
-4	24\\
-45.9958713325481	65.9958713325481\\
nan	nan\\
};

\addplot[area legend,solid,line width=1.0pt,draw=mycolor2,fill=mycolor3,fill opacity=0,forget plot]
table[row sep=crcr] {%
x	y\\
0	0\\
4	4\\
6.66666666666667	14.6666666666667\\
2.66666666666667	10.6666666666667\\
0	0\\
}--cycle;
\addplot [color=mycolor4,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0	0\\
};
\addplot [color=mycolor4,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0	0\\
};
\addplot [color=mycolor5,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.222222222222222	0.888888888888889\\
};
\addplot [color=mycolor5,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.222222222222222	0.888888888888889\\
};
\addplot [color=mycolor6,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.444444444444444	1.77777777777778\\
};
\addplot [color=mycolor6,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.444444444444444	1.77777777777778\\
};
\addplot [color=mycolor7,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.666666666666667	2.66666666666667\\
};
\addplot [color=mycolor7,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.666666666666667	2.66666666666667\\
};
\addplot [color=mycolor8,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-3.11111111111111	-0.444444444444445\\
};
\addplot [color=mycolor8,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.888888888888889	3.55555555555556\\
};
\addplot [color=mycolor2,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-2.88888888888889	0.444444444444445\\
};
\addplot [color=mycolor2,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.11111111111111	4.44444444444444\\
};
\addplot [color=mycolor9,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-2.66666666666667	1.33333333333333\\
};
\addplot [color=mycolor9,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.33333333333333	5.33333333333333\\
};
\addplot [color=mycolor10,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.55555555555556	-1.77777777777778\\
};
\addplot [color=mycolor10,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.55555555555556	6.22222222222222\\
};
\addplot [color=mycolor11,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.77777777777778	-0.888888888888889\\
};
\addplot [color=mycolor11,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.77777777777778	7.11111111111111\\
};
\addplot [color=mycolor12,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
2	0\\
};
\addplot [color=mycolor12,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2	8\\
};
\addplot [color=mycolor13,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.22222222222222	0.888888888888889\\
};
\addplot [color=mycolor13,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.22222222222222	8.88888888888889\\
};
\addplot [color=mycolor4,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.55555555555556	-2.22222222222222\\
};
\addplot [color=mycolor4,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.44444444444444	9.77777777777778\\
};
\addplot [color=mycolor5,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.33333333333333	1.33333333333333\\
};
\addplot [color=mycolor5,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.33333333333333	1.33333333333333\\
};
\addplot [color=mycolor6,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.55555555555556	2.22222222222222\\
};
\addplot [color=mycolor6,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.55555555555556	2.22222222222222\\
};
\addplot [color=mycolor7,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-2.22222222222222	-0.888888888888889\\
};
\addplot [color=mycolor7,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.77777777777778	3.11111111111111\\
};
\addplot [color=mycolor8,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-2	0\\
};
\addplot [color=mycolor8,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2	4\\
};
\addplot [color=mycolor2,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.77777777777778	0.888888888888888\\
};
\addplot [color=mycolor2,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.22222222222222	4.88888888888889\\
};
\addplot [color=mycolor9,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.55555555555556	1.77777777777778\\
};
\addplot [color=mycolor9,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.44444444444444	5.77777777777778\\
};
\addplot [color=mycolor10,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.33333333333333	2.66666666666667\\
};
\addplot [color=mycolor10,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.66666666666667	6.66666666666667\\
};
\addplot [color=mycolor11,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.88888888888889	-0.444444444444446\\
};
\addplot [color=mycolor11,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.88888888888889	7.55555555555555\\
};
\addplot [color=mycolor12,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.11111111111111	0.444444444444445\\
};
\addplot [color=mycolor12,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.11111111111111	8.44444444444444\\
};
\addplot [color=mycolor13,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.666666666666667	-2.66666666666667\\
};
\addplot [color=mycolor13,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.33333333333333	9.33333333333333\\
};
\addplot [color=mycolor4,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.444444444444445	-1.77777777777778\\
};
\addplot [color=mycolor4,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.55555555555556	10.2222222222222\\
};
\addplot [color=mycolor5,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.222222222222222	-0.888888888888889\\
};
\addplot [color=mycolor5,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.77777777777778	11.1111111111111\\
};
\addplot [color=mycolor6,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.33333333333333	-1.33333333333333\\
};
\addplot [color=mycolor6,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.66666666666667	2.66666666666667\\
};
\addplot [color=mycolor7,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-1.11111111111111	-0.444444444444445\\
};
\addplot [color=mycolor7,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
2.88888888888889	3.55555555555556\\
};
\addplot [color=mycolor8,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.888888888888889	0.444444444444445\\
};
\addplot [color=mycolor8,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.11111111111111	4.44444444444444\\
};
\addplot [color=mycolor2,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.666666666666667	1.33333333333333\\
};
\addplot [color=mycolor2,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.33333333333333	5.33333333333333\\
};
\addplot [color=mycolor9,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.444444444444445	2.22222222222222\\
};
\addplot [color=mycolor9,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.55555555555556	6.22222222222222\\
};
\addplot [color=mycolor10,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-0.222222222222222	3.11111111111111\\
};
\addplot [color=mycolor10,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
3.77777777777778	7.11111111111111\\
};
\addplot [color=mycolor11,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
-4	0\\
};
\addplot [color=mycolor11,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
4	8\\
};
\addplot [color=mycolor12,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.222222222222221	-3.11111111111111\\
};
\addplot [color=mycolor12,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
4.22222222222222	8.88888888888889\\
};
\addplot [color=mycolor13,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.444444444444445	-2.22222222222222\\
};
\addplot [color=mycolor13,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
4.44444444444444	9.77777777777778\\
};
\addplot [color=mycolor4,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.666666666666666	-1.33333333333333\\
};
\addplot [color=mycolor4,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
4.66666666666667	10.6666666666667\\
};
\addplot [color=mycolor5,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
0.888888888888889	-0.444444444444445\\
};
\addplot [color=mycolor5,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
4.88888888888889	11.5555555555556\\
};
\addplot [color=mycolor6,line width=1.3pt,only marks,mark=o,mark options={solid},forget plot]
  table[row sep=crcr]{%
1.11111111111111	0.444444444444443\\
};
\addplot [color=mycolor6,mark size=2.0pt,only marks,mark=*,mark options={solid},forget plot]
  table[row sep=crcr]{%
5.11111111111111	12.4444444444444\\
};
\node[below right, align=left, text=mycolor2]
at (axis cs:5,8) {$\mathcal{P}( \mathbf{G}_{\textrm{c}} \mathbf{M} )$};
\end{axis}
\end{tikzpicture}}
